Representative Language Generation

We introduce "representative generation," extending the theoretical framework for generation proposed by Kleinberg et al. (2024) and formalized by Li et al. (2024), to additionally address diversity and bias concerns in generative models. Our notion requires outputs of a generative model to proportionally represent groups of interest from the training data. We characterize representative uniform and non-uniform generation, introducing the "group closure dimension" as a key combinatorial quantity. For representative generation in the limit, we analyze both information-theoretic and computational aspects, demonstrating feasibility for countably infinite hypothesis classes and collections of groups under certain conditions, but proving a negative result for computability using only membership queries. This contrasts with Kleinberg et al.'s (2024) positive results for standard generation in the limit. Our findings provide a rigorous foundation for developing more diverse and representative generative models.

==> query_imposs_discussion.tex <==
Before providing the proof of Lemma~\ref{lem:gil-query-impossibility}, we provide some additional discussion of the result and comparison to the positive result of~\ifbool{arxiv}{\cite}{\citet}{kleinberg2024language}.

The algorithm of~\ifbool{arxiv}{\cite}{\citet}{kleinberg2024language} that generates in the limit using only a finite number of membership queries at each step crucially relies on the UUS assumption, in particular the fact that finding an element from $\supp{h} \setminus x_{1:t}$ is always possible because $|\supp{h}| = \infty$, and thus one can simply enumerate the elements of $\calX$ until an unseen point is encountered. In the case of representative generation, however, a generator may need to generate from $(\supp{h} \cap A_i) \setminus x_{1:t}$, which is not always guaranteed to be infinite, making this problem a lot more difficult. We note that in the case where $\calA$ partitions $\calX$, if we made the strong assumption that $\supp{h} \cap A_i$ is either empty or has infinite size for all $A_i \in \calA$ and $h \in \calH$, then this would be similar to the assumption made by \ifbool{arxiv}{\cite}{\citet}{kleinberg2024language}, and we could use membership queries to generate with representation using an algorithm almost identical to their membership-query algorithm. 

However, the Lemma~\ref{lem:finite-supp-imposs} shows that weakening this assumption to allow for groups with finite intersection with hypotheses in $\calH$ introduces some inherent difficulty. In particular, no algorithm that works even just for very simple, finite pairs of $\calH$ and $\calA$ can generate in the limit with representation using only membership queries. 

With this in mind, we present the proof below.
